Improved Surrogates in Inertial Confinement Fusion with Manifold and Cycle Consistencies

Neural networks have become very popular in surrogate modeling because of their ability to characterize arbitrary, high dimensional functions in a data driven fashion. This paper advocates for the training of surrogates that are consistent with the physical manifold -- i.e., predictions are always physically meaningful, and are cyclically consistent -- i.e., when the predictions of the surrogate, when passed through an independently trained inverse model give back the original input parameters. We find that these two consistencies lead to surrogates that are superior in terms of predictive performance, more resilient to sampling artifacts, and tend to be more data efficient. Using Inertial Confinement Fusion (ICF) as a test bed problem, we model a 1D semi-analytic numerical simulator and demonstrate the effectiveness of our approach. Code and data are available at https://github.com/rushilanirudh/macc/

==> related.tex <==
%%
Neural networks have become very a very popular tool in building surrogate models for a wide range of scientific simulators in the recent few years such as in particle physics \cite{paganini2018calogan} or porous media flows \cite{zhu2018bayesian}. Their popularity is owed primarily to the fact that it is significantly faster and computationally more efficient to evaluate the neural network surrogate instead of the simulator. Additionally, the neural network also has other attractive properties such as differentiability that may make it easier to add into existing machine learning workflows. As a result there has been renewed interest in building better surrogates for scientific problems. These include incorporating known scientific constraints into the training process \cite{?,?,?,?}, or reducing dimensionality for better uncertainty quantification \cite{tripathy2018deep}.
